PIVOINE: Instruction Tuning for Open-world Information Extraction

We consider the problem of Open-world Information Extraction (Open-world IE), which extracts comprehensive entity profiles from unstructured texts. Different from the conventional closed-world setting of Information Extraction (IE), Open-world IE considers a more general situation where entities and relations could be beyond a predefined ontology. More importantly, we seek to develop a large language model (LLM) that is able to perform Open-world IE to extract desirable entity profiles characterized by (possibly fine-grained) natural language instructions. We achieve this by finetuning LLMs using instruction tuning. In particular, we construct INSTRUCTOPENWIKI, a substantial instruction tuning dataset for Open-world IE enriched with a comprehensive corpus, extensive annotations, and diverse instructions. We finetune the pretrained BLOOM models on INSTRUCTOPENWIKI and obtain PIVOINE, an LLM for Open-world IE with strong instruction-following capabilities. Our experiments demonstrate that PIVOINE significantly outperforms traditional closed-world methods and other LLM baselines, displaying impressive generalization capabilities on both unseen instructions and out-of-ontology cases. Consequently, PIVOINE emerges as a promising solution to tackle the open-world challenge in IE effectively.

==> case_tables.tex <==
\begin{xltabular}{\textwidth}{|l|X|}
\caption{A sample long table.} \label{tab:long} \\
\modelname-7b Output & \\
GPT-4 Input & \makecell[l]{The following are information of an entity pair and a set of evidence paragraphs describing their relations.
\\\\
[head entity] Find It on the Wings
[head type] Album
[head description] album by Sandi Patty
[head aliases] 
\\\\
[tail entity] Sandi Patty
[tail type] Human
[tail description] American Christian music singer
[tail aliases] 
\\\\
[evidence paragraph 0] These Days is the twentieth studio album by Christian singer Sandi Patty. It was released on November 14, 2000 on Word Records. It is Patty's first new studio album of Christian material since 1997's "Artist of My Soul" and a return to her Christian AC/Pop sound reminiscent of "Find It on the Wings" and "Le Voyage" with songwriting contributions from Kathy Troccoli, Cindy Morgan, Scott Krippayne and Chris Eaton. Long-time producer Greg Nelson produces three tracks including a cover of Michael and Stormie Omartian's "One More Song for You," originally recorded by The Imperials. Production duties also handled by Brent Bourgeois, Phil Naish and Hal S. Batt on the Spanglish duet "Solo El Amor (Only Love)" with Latin singer Miguel Angel Guerra.
[head mention] Find It on the Wings
[tail mention] Sandi Patty
\\\\
[relation] The relation between head entity ``Find It on the Wings'' and tail entity ``Sandi Patty'' is ``performer''.
\\\\
Please judge whether this relation is correct based on your knowledge and these evidence paragraphs. Please provide indices of evidence paragraphs that can support your judgement and provide explanations.}
\\
\end{xltabular}
